Deadlock-free, Safe, and Decentralized Multi-Robot Navigation in Social Mini-Games via Discrete-Time Control Barrier Functions

We present an approach to ensure safe and deadlock-free navigation for decentralized multi-robot systems operating in constrained environments, including doorways and intersections. Although many solutions have been proposed that ensure safety and resolve deadlocks, optimally preventing deadlocks in a minimally invasive and decentralized fashion remains an open problem. We first formalize the objective as a non-cooperative, non-communicative, partially observable multi-robot navigation problem in constrained spaces with multiple conflicting agents, which we term as social mini-games. Formally, we solve a discrete-time optimal receding horizon control problem leveraging control barrier functions for safe long-horizon planning. Our approach to ensuring liveness rests on the insight that \textit{there exists barrier certificates that allow each robot to preemptively perturb their state in a minimally-invasive fashion onto liveness sets i.e. states where robots are deadlock-free}. We evaluate our approach in simulation as well on physical robots using F$1/10$ robots, a Clearpath Jackal, as well as a Boston Dynamics Spot in a doorway, hallway, and corridor intersection scenario. Compared to both fully decentralized and centralized approaches with and without deadlock resolution capabilities, we demonstrate that our approach results in safer, more efficient, and smoother navigation, based on a comprehensive set of metrics including success rate, collision rate, stop time, change in velocity, path deviation, time-to-goal, and flow rate.

==> algorithms/auction.tex <==
\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
\SetKwComment{Comment}{$\triangleright$\ }{$40$Hz cycle frequency}
\SetAlgoLined
\Input{Bids $b^i$ for each agent in $\mathcal{C}^t_{\mathcal{O}}$, initialize $q \gets 0$.}
\Output{$\sigma_\textsc{opt}$}
     Sort $\mathcal{C}^t_{\mathcal{O}}$ in decreasing order of $b^i$.\\
     \While{$\lvert \mathcal{C}^t_{\mathcal{O}} \rvert$ is non-empty:}{
         Increment $q$ by $1$.\\
         Let $a^i$ be the the first element in $\mathcal{C}^t_{\mathcal{O}}$.\\
         Set $\sigma^i = q$.\\
     $\mathcal{C}^t_{\mathcal{O}} \gets \mathcal{C}^t_{\mathcal{O}} \setminus \{a^i\}$.\\
    }
     return $\sigma_\textsc{opt} = \sigma^1\sigma^2 \ldots \sigma_{\lvert \mathcal{C}^t_{\mathcal{O}} \rvert}$\\
% \begin{enumerate}
%     \item Given set $\mathcal{C}^t_{\mathcal{O}}$ of agents conflicted over state $\mathcal{O}$ at time $t$ and their corresponding bids $b^i$, initialize $q \gets 0$.  \label{algo: Algorithm}
%     \item Sort $\mathcal{C}^t_{\mathcal{O}}$ in decreasing order of $b^i$.
%     \item Do the following for $\lvert \mathcal{C}^t_{\mathcal{O}} \rvert$ steps:
%     \begin{enumerate}
%         \item Increment $q$ by $1$.
%         \item Let $a^i$ be the the first element in $\mathcal{C}^t_{\mathcal{O}}$.
%         \item Set $\sigma^i = q$.
%         \item $\mathcal{C}^t_{\mathcal{O}} \gets \mathcal{C}^t_{\mathcal{O}} \setminus \{a^i\}$.
%     \end{enumerate}
%     \item Repeat steps $1-3$ while $\mathcal{C}^t_{\mathcal{O}}$ is non-empty. 
%     \item return $\sigma_\textsc{opt} = \sigma^1\sigma^2 \ldots \sigma_{\lvert \mathcal{C}^t_{\mathcal{O}} \rvert}$
% \end{enumerate}
\caption{Auction algorithm}
\label{algo: auction}
% \vspace{-10pt}
\end{algorithm}

==> algorithms/kinodynamic.tex <==
\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
\SetKwComment{Comment}{$\triangleright$\ }{$40$Hz cycle frequency}
\SetAlgoLined
\Input{$\sigma_\textsc{opt} = \sigma^1\sigma^2 \ldots \sigma_{\lvert \mathcal{C}^t_{\mathcal{O}} \rvert}$}
\Output{$\Xi^i_{\sigma_i}$}

\uIf{$\sigma^i = 1$}{
$v_\textrm{max}$ = \texttt{V\_MAX}
}
\Else{$v_\textrm{max}=$ \texttt{V\_MAX}/$\sigma^i$}

\caption{Retrieving kinodynamic constraints}
\label{algo: kino}
% \vspace{-10pt}
\end{algorithm}

==> images/CBF+Perturb_VS_CBF.tex <==
\begin{figure*}[t]
\centering
   \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/nongame1_edited.jpg}
    \caption{Initial time step}
    \label{fig: game1}
  \end{subfigure}
  %
 \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/game2_edited.jpg}
    \caption{The blue agent slows down}
    \label{fig: game2}
  \end{subfigure}
  %
\begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/game3_edited.jpg}
    \caption{The blue agent yields}
    \label{fig: game3}
  \end{subfigure}
    %
   \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/game4_edited.jpg}
    \caption{The blue agent follows the red.}
    \label{fig: game4}
  \end{subfigure}
  %
     \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/nongame1_edited.jpg}
    \caption{Initial time step}
    \label{fig: nongame1}
  \end{subfigure}
  %
 \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/nongame2_edited.jpg}
    \caption{Both agents move together}
    \label{fig: nongame2}
  \end{subfigure}
  %
\begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/nongame3_edited.jpg}
    \caption{Both agents enter a deadlock}
    \label{fig: nongame3}
  \end{subfigure}
    %
   \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/nongame4_edited.jpg}
    \caption{Deadlock scenario}
    \label{fig: nongame4}
  \end{subfigure}
  %
    \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/intersection_game_1_edited.jpg}
    \caption{Initial time step}
    \label{fig: game1_inter}
  \end{subfigure}
  %
 \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/intersection_game_2_edited.jpg}
    \caption{The blue agent slows down}
    \label{fig: game2_inter}
  \end{subfigure}
  %
\begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/intersection_game_3_edited.jpg}
    \caption{The blue agent yields}
    \label{fig: game3_inter}
  \end{subfigure}
    %
   \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/intersection_game_4_edited.jpg}
    \caption{The blue agent crosses.}
    \label{fig: game4_inter}
  \end{subfigure}
  %
     \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/intersection_ng_1_edited.jpg}
    \caption{Initial time step}
    \label{fig: nongame1_inter}
  \end{subfigure}
  %
 \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/intersection_ng_2_edited.jpg}
    \caption{Both agents move together}
    \label{fig: nongame2_inter}
  \end{subfigure}
  %
\begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/intersection_ng_3_edited.jpg}
    \caption{Both agents enter a deadlock}
    \label{fig: nongame3_inter}
  \end{subfigure}
    %
   \begin{subfigure}[h]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/PySim/intersection_ng_4_edited.jpg}
    \caption{Deadlock scenario}
    \label{fig: nongame4_inter}
  \end{subfigure}
\caption{\textbf{Liveness via Game-Theoretic Control Barrier Functions:} \textit{(doorway)} Figures~\ref{fig: game1},~\ref{fig: game2},~\ref{fig: game3},~\ref{fig: game4} show that the blue agent yields to the red agent without stopping and smoothly follows the red agent through. In Figures~\ref{fig: nongame1},~\ref{fig: nongame2},~\ref{fig: nongame3},~\ref{fig: nongame4}, both agents get stuck due to a lack of deadlock resolution. Similar observation in the intersection scenario. \textit{Conclusion:} Our game-theoretic controller presented in Section~\ref{sec: GT-resolution} encourages queue formation thereby resolving a deadlock situation in a distributed and smooth manner.} 
  \label{fig: PySim}
  % \vspace{-10pt}
\end{figure*}  


==> images/RVO/rvo.tex <==
\begin{figure}[t]
\centering
   \begin{subfigure}[h]{0.49\columnwidth}
    \includegraphics[width=\textwidth]{images/RVO/RVO_collision_doorway.png}
    \caption{Reciprocal Velocity Obstacles}
    \label{fig: rvo1}
  \end{subfigure}
  %
 % \begin{subfigure}[h]{0.32\textwidth}
 %    \includegraphics[width=\textwidth]{images/RVO/RVO_gapsize_doorway.png}
 %    \caption{Reciprocal Velocity Obstacles}
 %    \label{fig: rvo2}
 %  \end{subfigure}
  %
% \begin{subfigure}[h]{0.32\textwidth}
%     \includegraphics[width=\textwidth]{images/RVO/RVO_velocity_doorway.png}
%     \caption{Reciprocal Velocity Obstacles}
%     \label{fig: rvo3}
%   \end{subfigure}
    %
   \begin{subfigure}[h]{0.49\columnwidth}
    \includegraphics[width=\textwidth]{images/SVO/SF_collision_doorway.png}
    \caption{Social Forces}
    \label{fig: sf1}
  \end{subfigure}
  %
%  \begin{subfigure}[h]{0.32\textwidth}
%     \includegraphics[width=\textwidth]{images/SVO/SF_gapsize_doorway.png}
%     \caption{Social Forces}
%     \label{fig: sf2}
%   \end{subfigure}
%   %
% \begin{subfigure}[h]{0.32\textwidth}
%     \includegraphics[width=\textwidth]{images/SVO/SF_velocity_doorway.png}
%     \caption{Social Forces}
%     \label{fig: sf3}
%   \end{subfigure}
\caption{\textbf{Comparing with crowd simulation and collision avoidance models:} Measuring the time to goal and number of collisions with respect to number of agents for Reciprocal Velocity Obstacles (RVO)~\cite{rvo, orca} and Social Forces~\cite{socialforces}.}
  \label{fig: rvo_results}
  \vspace{-10pt}
\end{figure}  

==> images/cover/cover.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[h]{0.485\columnwidth}
\includegraphics[width = \columnwidth]{images/cover/ours1.jpg}   
    \caption{Initial time step}
    \label{fig: b1}
    \end{subfigure}
    %
    \begin{subfigure}[h]{0.485\columnwidth}
\includegraphics[width = \columnwidth]{images/cover/baseline2.jpg}   
    \caption{Collision}
    \label{fig: b2}
    \end{subfigure}
    %
     \begin{subfigure}[h]{0.485\columnwidth}
\includegraphics[width = \columnwidth]{images/cover/ours1.jpg}   
    \caption{Initial time step}
    \label{fig: o1}
    \end{subfigure}
    %
    \begin{subfigure}[h]{0.485\columnwidth}
\includegraphics[width = \columnwidth]{images/cover/ours2.jpg}   
    \caption{Queue formation}
    \label{fig: o2}
    \end{subfigure}
    \caption{\textbf{Fully decentralized multi-agent social navigation:} The mode \texttt{GAME=true} indicates that the cars are on a collision course. \textit{(top)} Figures~\ref{fig: b1} and~\ref{fig: b2} depict two F$1/10$ cars at the initial time-step and when they collide at the gap in the absence of any form of safety certificates. \textit{(bottom)} Figures~\ref{fig: o1} and~\ref{fig: o2} depict the same configurations but using game-theoretic safety barrier certificates, both cars independently choose \textit{safe} and \textit{efficient} control inputs resulting in a queue to safely navigate the doorway.}
    \label{fig: mini-games}
    \vspace{-10pt}
\end{figure}

==> images/smg60_tikz.tex <==
% \begin{tikzpicture}[scale=1]
%     % Nodes for agents
%     \node[circle, draw=green!50!black, fill=green!30, minimum size=1cm] (i) at (0,0) {};
%     \node[circle, draw=green!50!black, fill=green!30, minimum size=1cm] (j) at (5,0) {};
%     \node[circle, draw=red!50!black, fill=red!30, minimum size=0.7cm] (goal) at (2.5,2.5) {};
    
%     % Labels for agents and goal
%     \node[below=4mm] at (i) {\textbf{agent $i$}};
%     \node[below=4mm] at (j) {\textbf{agent $j$}};
%     \node[above=4mm] at (goal) {\textbf{$Q$}};
    
%     % Connecting lines
%     \draw[thick, blue] (i) -- (goal) node[midway, sloped, above] {\large $d$};
%     \draw[thick, blue] (j) -- (goal) node[midway, sloped, above] {\large $d$};
%     \draw[thick, blue, ->] (i) -- (j) node[midway, below] {\large ${P}_{ij}$};
    
%     % Velocity vectors (green and purple)
%     \draw[->, green!70!black, thick] (i) -- ++(45:1) node[above=1mm, left=1mm] {\large ${v}^i_t$};
%     \draw[->, purple, thick] (i) -- ++(30:1) node[above=1mm, right=2mm] {\large ${v}^i_t \cdot \sec(\theta)$};
%     \draw[->, green!70!black, thick] (j) -- ++(135:1) node[above=0.5mm, right=1mm] {\large ${v}^j_t$};
%     \draw[->, purple, thick] (j) -- ++(150:1) node[below=.1mm, left=2mm] {${v}^j_t 
%     \cdot \sec(\theta')$};
    
%     % Angles (theta between blue and green arrows)
%     \draw[thick, blue!50] (i) ++(0:0.5) arc[start angle=0, end angle=45, radius=0.5];
%     \node at ($(i) + (15:0.7)$) {\large $\theta= \frac{\pi}{3}$};
%     \draw[thick, blue!50] (j) ++(180:0.5) arc[start angle=180, end angle=135, radius=0.5];
%     \node at ($(j) + (165:0.7)$) {\large $\theta= \frac{\pi}{3}$};
    
%     % New angles (theta' between green and purple arrows)
%     \draw[thick, purple!50] (i) ++(45:0.4) arc[start angle=45, end angle=30, radius=0.4];
%     \node at ($(i) + (37.5:0.6)$) {\large $\theta'$};
%     \draw[thick, purple!50] (j) ++(135:0.4) arc[start angle=135, end angle=150, radius=0.4];
%     \node at ($(j) + (142.5:0.6)$) {\large $\theta'$};
    
%     % Additional text
%     \node[below=0.8cm] at ($(i)!0.5!(j)$) {\textcolor{red}{\large $\theta - \theta' = 45$}};
% \end{tikzpicture}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\linewidth]{images/smg30.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}

==> sections/approach.tex <==
% \section{Deadlock Resolution}
% \label{sec: main_approach}

We solve the multi-robot navigation problem~\eqref{def: best_response} for the discrete-time system~\eqref{eq: control_affine_dynamics} in a decentralized fashion. Each robots solves~\eqref{eq: best_response_example} in a receding horizon fashion using an MPC. At each time step $t$ for the $i^\textrm{th}$ robot, the MPC controller solves the constrained finite-time optimal control problem~\eqref{eq: best_response_example} with horizon $T$. The optimal solution at time $t$ is a sequence of inputs as $\Psi^{i,*} = [u^{i,*}_{t},u^{i,*}_{t+1} \ldots, u^{i,*}_{t+T-1}]$, $u^{i,*}_{t} \in \mathscr{U}^i_t$ for each $t$. Then, the first element of the optimizer vector is applied $u^i_t \gets u^{i,*}_t$. The constrained finite-time optimal control strategy~\eqref{eq: best_response_example} is repeated at time step $t+1$, based on the new state $x^i_{t+1}$, yielding a receding horizon control strategy. Note that the constraint~\eqref{eq: sub_coll} in~\eqref{eq: best_response_example} depends on the state of other robots. Therefore, robots solve~\eqref{eq: best_response_example} in an asynchronous fashion; on the $i^\textrm{th}$ robot's turn, it treats all other robots as static obstacles that are incorporated into the CBF for the $i^\textrm{th}$ robot.

\subsection{Safety}
We model safety in Equation~\eqref{eq: sub_coll} in the context of set invariance using CBFs. The discrete CBF safety constraint is given by,

\begin{equation}
    \Delta h_s^i\left(x^i_{t},  u^i_t\right) = h_s^i\left(x^i_{t+1}\right) - h_s^i\left(x^i_{t}\right)
    \label{eq: discrete_barrier_func}
\end{equation}

where $h_s^i\left(x^i_{t}\right)$ is chosen as an obstacle avoidance barrier function (more details in Section~\ref{subsec: exp_setup}). Let $\mathscr{U}^i_t \subset \mathcal{U}^i$ be the set of collision-free controls for robot $i$ such that the following holds,

\begin{equation}
\Delta h^i_s\left(x^i_t,  u^i_t\right) \geq -\gamma h_s^i\left(x^i_t\right)
    \label{eq: discrete_barrier_func}
\end{equation}

where $\gamma$ is chosen as as a scalar for simplicity.  We refer the reader to Zeng et al.~\cite{zeng2021safety_cbf_mpc} for more details on the single-agent MPC-CBF formulation.
% In practice, the optimization problem~\eqref{eq: best_response_example} can be solved optimally (if a solution is reached) via a Dynamic Window Approach (DWA)~\cite{dwa}, Model predictive Controller (MPC)~\cite{park2012robot}, Control Barrier Functions (CBF)~\cite{ames2019control}, among others. Let $\mathscr{U}^i_t \subset \mathcal{U}^i$ be the set of controls such that Equation~\eqref{eq: sub_coll} holds and robot $i$ is collision-free. Further, let $\pi^i \in \mathcal{K}$ refer to a chosen controller (MPC, DWA etc.) chosen by agent $i$, where $\mathcal{K}$ denotes the set of possible controllers.



==> tables/marl.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{crcccc}
    \toprule
    & Baseline & Success Rate & Coll. Rate & Stop Time & $\# \Delta$V \\
    \midrule
    \multirow{5}{*}{\rotatebox{90}{DOOR}} & CADRL~\cite{cadrl} & $32\pm3.125$ & $0.00\pm0.000$ & $222\pm2.749$ & $13\pm1.905$ \\
    & CADRL w. LSTM~\cite{cadrl-lstm} & $0\pm0.000$ & $0.12\pm0.000$ & $436\pm0.318$ & $36\pm3.042$ \\
    % & CADRL-DQN &&&& \\
    & CADRL-priority order~\cite{cadrl-lstm} & $44\pm2.993$ & $0.16\pm0.243$ & $617\pm1.803$ & $117\pm0.686$ \\
    % & Enforced Order-LSTM &&&& \\
    % & Any Order & $84\pm2.319$ & $0.32\pm0.586$ & $324\pm1.390$ & $51\pm0.294$ \\
    % & Any Order-LSTM &&&& \\
    & DWA & $4\pm0.244$ & $2.32\pm0.589$ & $166\pm4.496$ & $30\pm2.506$ \\
 %    & SNUPI~\cite{snupi} & $76\pm2.270$ & $0.17\pm0.012$ & $110\pm4.100$ & $6\pm1.111$ \\
 % & Game-theoretic QP-CBF~\cite{wang2017safety} & 100$\pm$0.000 & 0.00$\pm$0.000 & 25$\pm$4.235 & 2$\pm$0.000 \\
    \rowcolor{gray!25} & \textbf{Game-theoretic MPC-CBF} & \textbf{100$\pm$0.000} & \textbf{0.00$\pm$0.000} & \textbf{18$\pm$1.067} & \textbf{2$\pm$0.098} \\
    % & No Local &&&& \\
    \cmidrule{2-6}
    \multirow{5}{*}{\rotatebox{90}{INTER.}} & CADRL~\cite{cadrl} & $20\pm0.453$ & $1.20\pm0.634$ & $389\pm5.153$ & $28\pm1.141$ \\
    & CADRL w. LSTM~\cite{cadrl-lstm} & $28\pm2.527$ & $0.32\pm1.393$ & $267\pm6.453$ & $127\pm2.357$ \\
    % & CADRL-DQN &&&& \\
    & CADRL-priority order~\cite{cadrl-lstm} & $56\pm0.718$ & $0.80\pm0.894$ & $233\pm1.729$ & $104\pm5.041$ \\
    % & Enforced Order-LSTM &&&& \\
    % & Any Order & $28
        % &Enforced Order-LSTM &&&& \\
        % &Any Order &28&0.68&592&47 \\
        % &Any Order-LSTM &&&& \\
        % &Our Approach&44&0.05&640&97 \\
        &DWA&$16\pm 1.765$&$2.48 \pm 0.57$&$640 \pm 4.583$&$97 \pm 2.495$ \\
        % &SNUPI~\cite{snupi}&$96 \pm 3.342$&$0.14 \pm 0.003$&$139\pm 5.233$&$6 \pm 0.470$ \\ 
        % &Game-theoretic QP-CBF~\cite{wang2017safety}& 100$\pm$ 0.000&0.00$\pm$ 0.000&46$\pm$ 2.349&2$\pm$ 0.040 \\
        \rowcolor{gray!25}&\textbf{Game-theoretic MPC-CBF}& \textbf{100$\pm$ 0.000}&\textbf{0.00$\pm$ 0.000}&\textbf{27$\pm$ 0.140}&\textbf{0$\pm$ 0.000} \\
        % &No Local&&&& \\
         \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Comparing Game-theoretic MPC-CBF versus baselines \underline{without} deadlock resolution capabilities:} 
    % We compare with MARL baselines and DWA, which is a baseline method where only the local motion planner is used without scheduling. CADRL~\cite{cadrl} and its LSTM variant~\cite{cadrl-lstm} are state-of-the-art RL-based social navigation algorithms and Enforced Order uses sub-goal reward policies that encourage queue formation. 
    Navigation with game-theoretic deadlock resolution results in higher success rates and more efficient navigation in terms of fewer stop times and changes in velocity.}
    \label{tab: main_exps_marl}
    % \vspace{-15pt}
\end{table}



